Metal Artifact Reduction in 2D CT Images with Self-supervised Cross-domain Learning

The presence of metallic implants often introduces severe metal artifacts in the X-ray CT images, which could adversely influence clinical diagnosis or dose calculation in radiation therapy. In this work, we present a novel deep-learning-based approach for metal artifact reduction (MAR). In order to alleviate the need for anatomically identical CT image pairs (i.e., metal artifact-corrupted CT image and metal artifact-free CT image) for network learning, we propose a self-supervised cross-domain learning framework. Specifically, we train a neural network to restore the metal trace region values in the given metal-free sinogram, where the metal trace is identified by the forward projection of metal masks. We then design a novel FBP reconstruction loss to encourage the network to generate more perfect completion results and a residual-learning-based image refinement module to reduce the secondary artifacts in the reconstructed CT images. To preserve the fine structure details and fidelity of the final MAR image, instead of directly adopting CNN-refined images as output, we incorporate the metal trace replacement into our framework and replace the metal-affected projections of the original sinogram with the prior sinogram generated by the forward projection of the CNN output. We then use the filtered backward projection (FBP) algorithms for final MAR image reconstruction. We conduct an extensive evaluation on simulated and real artifact data to show the effectiveness of our design. Our method produces superior MAR results and outperforms other compelling methods. We also demonstrate the potential of our framework for other organ sites.

==> Related.tex <==
\section{Related Work}
\label{sec:relatedwork}

\subsection{Conventional Metal Artifact Reduction}
Metal artifact reduction is a long-standing problem in image reconstruction field. 
The previous metal artifact reduction approaches mainly address this problem  in X-ray projections (sinogram). 
%
The metal-affected regions in sinogram are corrected by modeling the underlying physical effects of imaging~\cite{hsieh2000iterative,kachelriess2001generalized,meyer2010empirical,park2015metal}.
For example, Park \etal~\cite{park2015metal}  proposed a new method to correct beam hardening artifacts caused by the presence of metal in polychromatic X-ray CT. 
%
However, the metal trace regions in sinogram are often severe corrupted and the above methods cannot achieve satisfactory results. 
%%
Therefore, the widely used MAR methods regard the metal-affected regions as missing and replace them with estimated values~\cite{kalender1987reduction,mehranian2013x}.
%
The early Linear interpolation (LI) approach~\cite{kalender1987reduction} filled the missing data by the linear interpolation of its neighboring unaffected data for each projection view, while it often introduces new artifacts near large metals, as interpolation cannot completely recover the metal trace information.
%
Meyer \etal~\cite{meyer2010normalized} improved the LI approach by generating a prior image with tissue processing and normalizing the projection with the forward projection of the prior image before interpolation.
 %%
Besides interpolation in projection (sinogram) domain, there are also some works focusing on designing new iterative reconstruction algorithms to construct artifact-free images from the unaffected or corrected projections~\cite{wang1996iterative,wang1999iterative,lemmens2008suppression,zhang2011metal}.
%%
\ylq{For example, XXX}
However, these iterative reconstruction methods often suffer from a large amount of computation and require proper hand-crafted regularizations. 


\subsection{Deep Learning Based Methods for MAR}
Plenty of deep learning methods have recently been proposed to conduct MAR in sinogram domain, image domain and jointly in two domains.
%%
Park~\etal employed a U-Net~\cite{ronneberger2015u} to correct metal-induced beam hardening in the projection domain~\cite{park2018ct} and image domain~\cite{park2017machine}, respectively, while 
Gjesteby~\etal developed a few deep learning based MAR methods that refine the performance of  NMAR, with deep learning in the projection domain~\cite{gjesteby2017deep} and image domain~\cite{gjesteby2017reducing,gjesteby2017deep}, respectively.
%
The CNN was used to help overcome residual errors from the NMAR. While their experiments demonstrated that CNN can improve the NMAR effectively, remaining artifacts are still considerable.
%%

More recently,  RL-ARCNN~\cite{huang2018metal} introduced residual learning into a deep convolutional neural network (CNN) and achieved better MAR performance than standard CNN. 
%
Gjesteby~\cite{gjesteby2018deep} employed a deep network to reduce
the secondary artifacts after the normalized MAR method with a perceptual loss.
% 
CNNMAR~\cite{zhang2018convolutional} uses CNN to generate prior images in the CT image domain to help the correction in the projection domain. Both DestreakNet and CNNMAR show significant improvements over the existing non-DNN based methods on synthesized datasets. cGANMAR~\cite{wang2018conditional} leverages generative adversarial networks (GANs) [13] to further improve the DNN- based MAR performance.
%%
There are also some works to utilize dual domain learning~\cite{lin2019dudonet,lyu2020dudonet}.
%%
 
